From Disagreement to Understanding: The Case for Ambiguity Detection in NLI

This position paper argues that annotation disagreement in Natural Language Inference (NLI) is not mere noise but often reflects meaningful variation, especially when triggered by ambiguity in the premise or hypothesis. While underspecified guidelines and annotator behavior contribute to variation, content-based ambiguity provides a process-independent signal of divergent human perspectives. We call for a shift toward ambiguity-aware NLI that first identifies ambiguous input pairs, classifies their types, and only then proceeds to inference. To support this shift, we present a framework that incorporates ambiguity detection and classification prior to inference. We also introduce a unified taxonomy that synthesizes existing taxonomies, illustrates key subtypes with examples, and motivates targeted detection methods that better align models with human interpretation. Although current resources lack datasets explicitly annotated for ambiguity and subtypes, this gap presents an opportunity: by developing new annotated resources and exploring unsupervised approaches to ambiguity detection, we enable more robust, explainable, and human-aligned NLI systems.

==> latex/figures/implicature-ambiguity.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,171); %set diagram left start at 0, and has height of 171

%Shape: Rectangle [id:dp8562264468207915] 
\draw   (18,15.5) -- (311,15.5) -- (311,117) -- (18,117) -- cycle ;
%Shape: Rectangle [id:dp5180894034191962] 
\draw  [fill={rgb, 255:red, 255; green, 242; blue, 204 }  ,fill opacity=1 ] (18,15.5) -- (311,15.5) -- (311,47) -- (18,47) -- cycle ;

% Text Node
\draw (164.13,84.75) node  [font=\fontsize{0.8em}{0.96em}\selectfont] [align=left] {\begin{minipage}[lt]{210.97pt}\setlength\topsep{0pt}
{\fontfamily{helvet}\selectfont \textbf{\textcolor[rgb]{0.29,0.56,0.89}{Premise}:} ``\textbf{It hopes to bring on another 25 or 35 people \ when the new building opens next fall.''}}\\{\fontfamily{helvet}\selectfont \textcolor[rgb]{0.96,0.65,0.14}{\textbf{Hypothesis}}: ``\textbf{They already have a waiting list for the new building.''}}
\end{minipage}};
% Text Node
\draw (180,33) node  [font=\fontsize{0.8em}{0.96em}\selectfont] [align=left] {\begin{minipage}[lt]{115.6pt}\setlength\topsep{0pt}
{\fontfamily{helvet}\selectfont \textbf{Implicature Ambiguity}}
\end{minipage}};


\end{tikzpicture}


==> latex/figures/temporal-reference-example.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,175); %set diagram left start at 0, and has height of 175

%Shape: Rectangle [id:dp558348468998719] 
\draw   (18,15.5) -- (311,15.5) -- (311,127) -- (18,127) -- cycle ;
%Shape: Rectangle [id:dp0014565741836105595] 
\draw  [fill={rgb, 255:red, 217; green, 234; blue, 211 }  ,fill opacity=1 ] (18,15.5) -- (311,15.5) -- (311,47) -- (18,47) -- cycle ;

% Text Node
\draw (164.63,88.25) node  [font=\fontsize{0.8em}{0.96em}\selectfont] [align=left] {\begin{minipage}[lt]{211.65pt}\setlength\topsep{0pt}
{\fontfamily{helvet}\selectfont \textbf{\textcolor[rgb]{0.29,0.56,0.89}{Premise}:} ``\textbf{You wake up one bright autumn morning and you’re halfway to the subway when you decide to walk to work instead.''}}\\{\fontfamily{helvet}\selectfont \textcolor[rgb]{0.96,0.65,0.14}{\textbf{Hypothesis}}: ``\textbf{You wake up early and decide to walk instead of take the subway.''}}
\end{minipage}};
% Text Node
\draw (180,33) node  [font=\fontsize{0.8em}{0.96em}\selectfont] [align=left] {\begin{minipage}[lt]{115.6pt}\setlength\topsep{0pt}
{\fontfamily{helvet}\selectfont \textbf{Temporal Reference}}
\end{minipage}};


\end{tikzpicture}

